Improving random walk rankings with feature selection and imputation

The Science4cast Competition consists of predicting new links in a semantic network, with each node representing a concept and each edge representing a link proposed by a paper relating two concepts. This network contains information from 1994-2017, with a discretization of days (which represents the publication date of the underlying papers). Team Hash Brown's final submission, \emph{ee5a}, achieved a score of 0.92738 on the test set. Our team's score ranks \emph{second place}, 0.01 below the winner's score. This paper details our model, its intuition, and the performance of its variations in the test set.

==> commented_out.tex <==
\begin{comment}
\section{Analysis}
\subsection{Ablation Analysis}

Various models with test scores: 
ef59, 0.9270788503013558 

score of hoprec truncatd at 0.5, with the second derivative features removed, logistic: 0.9246993728810569

0.9256107986837139 with 16-16-16
0.9259801986418433:  hoprec 0.5 truncate with (10, 10, 10, 10, 10) architecture. (deeper)
c15b
 [2021-11-11 01:25:15,937][INFO]start scoring of 1636589777-4212-55743.json [2021-11-11 01:25:15,991][INFO]1636589777-4212-55743.json has size 9.430780410766602MB [2021-11-11 01:25:17,864][INFO]Evaluation completed ok with score 0.9267829130451598 for 1636589777-4212-55743.json --- 0.9267 is this: 32 x 3 with dropout, train 10 times average. 
 
 3ed63
 [2021-11-11 02:25:14,733][INFO]start scoring of 1636593311-4212-20742.json [2021-11-11 02:25:14,765][INFO]1636593311-4212-20742.json has size 9.430780410766602MB [2021-11-11 02:25:16,584][INFO]Evaluation completed ok with score 0.9245862164230492 for 1636593311-4212-20742.json
 
 46177: downsample = 1, 13 x 5 with hoprec + warp. 0.9271.
2d2d: 16 x 5. 092713. (Slightly lower than 13 x 5)
0b77: 16 x 5. Just hoprec. 0.9261. Lower than with warp.


0b77
 [2021-11-11 07:33:32,878][INFO]start scoring of 1636611947-4212-99330.json [2021-11-11 07:33:35,295][INFO]1636611947-4212-99330.json has size 9.430780410766602MB [2021-11-11 07:33:37,157][INFO]Evaluation completed ok with score 0.9261477481981635 for 1636611947-4212-99330.json
 0.92614774819816 
2d2d
 [2021-11-11 07:33:28,250][INFO]start scoring of 1636610725-4212-14173.json [2021-11-11 07:33:28,343][INFO]1636610725-4212-14173.json has size 9.430780410766602MB [2021-11-11 07:33:30,232][INFO]Evaluation completed ok with score 0.9271345745027604 for 1636610725-4212-14173.json
Notes  0.92713457450276 
16 x 5 downsample = 1, hoprec + warp
46177
 [2021-11-11 07:33:22,661][INFO]start scoring of 1636610201-4212-57429.json [2021-11-11 07:33:24,856][INFO]1636610201-4212-57429.json has size 9.430780410766602MB [2021-11-11 07:33:27,583][INFO]Evaluation completed ok with score 0.9271801563178601 for 1636610201-4212-57429.json
 
 





\begin{table}
\centering
\begin{tabular}{||c | c c c c||} 
\hline
& \multicolumn{2}{c}{Val} & \multicolumn{2}{c||}{Test} \\
Hidden size & EM & F1 & EM & F1\\
\hline\hline
128  & 0.326 & 0.435 & 0.303 & 0.422\\
256  & 0.332 & 0.445 & 0.321 & 0.449\\
512  & 0.329 & 0.447 & 0.319 & 0.441\\
\hline
\end{tabular}
\caption{Comparison of performances of the final model with different sizes of the hidden layers.}
\label{tab:hidden size comparison}
\end{table}
\end{comment}



\begin{comment}
Full table with train/val
\begin{table}
\centering
\begin{tabular}{||c|ccc||} 
\hline
Models & Train & Val & Test\\ %\multicolumn{2}{c}{Train} & \multicolumn{2}{c||}{Test} \\
\hline\hline 
HOPREC baseline & 0.85385 & 0.83386 & 0.89 \\
Logistic with all features & 0.8996  & 0.8997 & 0.9250 \\
Logistic without second derivatives & 0.90065, & 0.90187 & 0.9247 \\ %ddec
MLP (32x3) & XXX & XXX & 0.92678 \\
MLP (13x5) & 0.90233  & 0.90235 & \textbf{0.92739} \\
MLP (13x5) + WARP & 0.92718 \\ %46177
MLP (13x5) + dropout & xxx & xxx & 0.9257 \\ 
MLP (13x5) + SAGE & xxx & xxx & 0.92605 \\ %3ed63
MLP (13x5) + GCN & xxx & xxx & 0.9252 \\ %ba258 

\hline 
\end{tabular}
\vskip12pt
\caption{Performances of different models on the test set.}
\label{tab:overall comparison}
\end{table}
\end{comment}


%Among the 40 features of this simplified model, the features with the highest odds ratios above 1 are: the max PageRank of the two nodes (190), HOPREC score (81.82), and the max outdegree of the two nodes (2.17).
%Meanwhile, features with the lowest odds ratios below 1 are: the max degree of the two nodes (0.021), the max number of papers of the two nodes (0.4), and the min degree of the two nodes (0.45). 

%Features with lowest weights are XXX. 
